Robotic Perception of Object Properties using Tactile Sensing

The sense of touch plays a key role in enabling humans to understand and interact with surrounding environments. For robots, tactile sensing is also irreplaceable. While interacting with objects, tactile sensing provides useful information for the robot to understand the object, such as distributed pressure, temperature, vibrations and texture. During robot grasping, vision is often occluded by its end-effectors, whereas tactile sensing can measure areas that are not accessible by vision. In the past decades, a number of tactile sensors have been developed for robots and used for different robotic tasks. In this chapter, we focus on the use of tactile sensing for robotic grasping and investigate the recent trends in tactile perception of object properties. We first discuss works on tactile perception of three important object properties in grasping, i.e., shape, pose and material properties. We then review the recent development in grasping stability prediction with tactile sensing. Among these works, we identify the requirement for coordinating vision and tactile sensing in the robotic grasping. To demonstrate the use of tactile sensing to improve the visual perception, our recent development of vision-guided tactile perception for crack reconstruction is presented. In the proposed framework, the large receptive field of camera vision is first leveraged to achieve a quick search of candidate regions containing cracks, a high-resolution optical tactile sensor is then used to examine these candidate regions and reconstruct a refined crack shape. The experiments show that our proposed method can achieve a significant reduction of mean distance error from 0.82 mm to 0.24 mm for crack reconstruction. Finally, we conclude this chapter with a discussion of open issues and future directions for applying tactile sensing in robotic tasks.

==> aboutauthors.tex <==
\begin{frontmatter}
\chapter*{Biography}
\end{frontmatter}

\begin{biography}

  \section*{Sir Stanley Davidson (1894--1981)}

  One or more blank lines denote the end of a paragraph.  The ends of\index{index}
  words and sentences are marked by spaces. It doesn't matter how many
  spaces you type; one is as good as 100.  The end of a line counts as
  a space.

\end{biography}


==> chapter2.tex <==
\cleardoublepage

\begin{frontmatter}
\chapter{Chapter Title\footnote{This is chapter footnote}}\label{chap2}
\subchapter{Chapter Subtitle}

\begin{aug}
\author[addressrefs={ad1,ad2}]%
  {\fnm{Firstname}   \snm{Surname}}%
  %{\fnm{Firstname}   \snm{Surname}\footnote{This is author footnote}}%
\author[addressrefs={ad2}]%
 {\fnm{Firstname} \snm{Surname}}%
\address[id=ad1]%
  {Short Address}%
\address[id=ad2]%
  {Long Address}%
\end{aug}


% \minitoc

%
\begin{chapterpoints}%[Chapter Points]
\item The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.

\item The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.
\end{chapterpoints}

\begin{dispquote}

  The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.

  The ends of words and sentences are marked by spaces. It doesn't
  matter how many spaces you type; one is as good as 100.  The end of
  a line counts as a space.
  
  \source{Name}

\end{dispquote}

\end{frontmatter}


\section{Section title}\label{sec2.1}


==> contributors.tex <==
%% Contributors list %%
\begin{frontmatter}
\chapter*{Contributors}
\end{frontmatter}

\begin{contributorslist}
  \name{Greg N. Gregoriou} is Professor of Finance in the School of
  Business and Economics at State University of New York at
  Plattsburgh. He obtained his Ph.D. (finance) from the University of
  Quebec at Montreal and is hedge-fund editor for the peer-reviewed
  scientific journal Derivatives Use, Trading and Regulation and
  editorial board member for the Journal of Wealth Management, and the
  Journal of Risk and Financial Institutions. He has written more than
  50 articles on hedge funds and managed futures in various U.S. and
  U.K. peer-reviewed publications, including (among others) the
  Journal of Portfolio Management, Journal of Derivatives Accounting,
  Journal of Futures Markets, European Journal of Operational
  Research, Annals of Operations Research, European Journal of
  Finance, and Journal of Asset Management. He has edited 18 books for
  Elsevier, Wiley, Palgrave-MacMillan, and Risk and has coauthored one
  book for Wiley.

  \name{Donald F. Dansereau} Department of Psychology, Texas Christian
  University, Fort worth, Texas

  \name{Ruth Garner} Department of Educational Psychology, Texas A \&
  M University, College Station, Texas
\end{contributorslist}



==> dedication.tex <==
  %% Dedication page
\begin{dedication}
  %% Dedication
  %% can be few\\
  %% lines long
\end{dedication}


==> listoffigures.tex <==
\begin{frontmatter}
\chapter*{List of Figures}
\end{frontmatter}

\listoffigures


==> part.tex <==
\cleardoublepage
\begin{frontmatter}
%\part{}
\end{frontmatter}

% Text ...


==> part1.tex <==
\begin{frontmatter}
\part{Part title}\label{part1}
\end{frontmatter}

% Text ...


==> preface.tex <==
\cleardoublepage
\begin{frontmatter}
\chapter*{Preface}%
%\addcontentsline{toc}{schapter}{Preface}
\end{frontmatter}


 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

 The ends of words and sentences are marked by spaces. It doesn't
 matter how many spaces you type; one is as good as 100.  The end of
 a line counts as a space.

\source%
{%
  \author{Name}\\%
  % \address{Location}\\%
  % \date{Month Year}%
}


==> tableofcontents.tex <==
%% Table of Contents %%
\begin{frontmatter}
\chapter*{Contents}
\end{frontmatter}

\tableofcontents


==> titlepage.tex <==
%% Title Page %%
\begin{titlepage}%
  \begin{titlepagerule}
    \title{Book title}
    %\subtitle{Book Subtitle}
    %\volume{2}
  \end{titlepagerule}

  \edition{2nd edition}

%  \editedby{Edited by}

  \author{Author Firstname  Surname}
  \address{Author Address\\Department of Chemistry\\University of Florida}

  \author{Author Firstname  Surname}
  \address{Author Address}
\end{titlepage}

